Case Study: Leveraging GenAI to Build AI-based Surrogates and Regressors for Modeling Radio Frequency Heating in Fusion Energy Science

This work presents a detailed case study on using Generative AI (GenAI) to develop AI surrogates for simulation models in fusion energy research. The scope includes the methodology, implementation, and results of using GenAI to assist in model development and optimization, comparing these results with previous manually developed models.

==> plots_current.tex <==

% generate a 3x3 grid of images
% rows are methods
% cols are best, median, worst MSE

\begin{figure*}

     \centering
    % first row: RFR full: good, avg, poor
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_full_curtor_good_1917.png}
         \label{fig:rfr_current_good}
     \end{subfigure}
     \hfill
       \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_full_curtor_avg_1526.png}
         \label{fig:rfr_current_avg}
     \end{subfigure}
     \hfill
        \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_full_curtor_poor_53.png}
         \label{fig:rfr_current_poor}
     \end{subfigure}
     \\
      % second row: RFR reduced: good, avg, poor
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_reduced_curtor_good_1917.png}
         \label{fig:rfr_reduced_current_good}
     \end{subfigure}
     \hfill
       \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_reduced_curtor_avg_1526.png}
         \label{fig:rfr_reduced_current_avg}
     \end{subfigure}
     \hfill
        \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/RFR_reduced_curtor_poor_53.png}
         \label{fig:rfr_current_poor}
     \end{subfigure}
     \\
     % third row: MLP full, good, avg, poor
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_full_curtor_good_1917.png}
         \label{fig:mlp_current_good}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_full_curtor_avg_1526.png}
         \label{fig:rfr_current_avg}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_full_curtor_poor_53.png}
         \label{fig:mlp_current_avg}
     \end{subfigure}
     \\
% fourth row: MLP reduced, good, avg, poor
           \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_reduced_curtor_good_1917.png}
         \label{fig:mlp_reduced_current_good}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_reduced_curtor_avg_1526.png}
         \label{fig:rfr_reduced_current_avg}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/MLP_reduced_curtor_poor_53.png}
         \label{fig:mlp_reduced_current_avg}
     \end{subfigure}
            \caption{For the variable current drive, comparison of model outputs for RFR with all features (first row), RFR with partial features (second row), MLP with all features (third row), and MLP with reduced features (bottom row). The left column shows typical "good" model accuracy, the middle column shows an "average" model accuracy, and the right column shows a "poor" model accuracy. Results for the variable \emph{powers} are similar and omitted for brevity. In these charts, the x-axis is the set of targets, or output values, produced by the model. The y-axis is the numerical value of each of these output values.
        }
        \label{fig:current_good_avg_poor}

\end{figure*}



==> table_genai_uses.tex <==
\begin{table*}[]
    \centering
    \def\arraystretch{1.25}% create some spacing between rows
    \begin{tabular}{p{1.5in}p{1.5in}p{2.5in}}
    Processing stage & Role of \genai{} & Prompts and responses \\
%
\hline 
    Exploratory data analysis & Describe key concepts & prompt here \\
%
Initial model development & role & prompt \\
%
Exploratory model analysis & role & prompt \\
%
Model optimization and cross-validation & Describe process for k-fold CV & prompt \\
  & Provide code templates for k-fold CV & prompt goes here \\
%
    \end{tabular}
    \caption{Role of \genai{} at various stages of model construction, optimization, and evaluation.}
    \label{tab:role_of_genai}
\end{table*}

==> table_results_timings.tex <==
\begin{table*}[h!]
     \centering
    \begin{tabular}{l|cccc|cccc}
    \toprule
    & \multicolumn{4}{c|}{5-Fold CV} & \multicolumn{4}{c}{Test (hold-out data)} \\
    & \multicolumn{2}{c}{Current} & \multicolumn{2}{c|}{Powers} & \multicolumn{2}{c}{Current} & \multicolumn{2}{c}{Powers} \\
    Method & Train & Inference & Train & Inference & Train & Inference & Train & Inference \\
    \midrule
    MLP sklearn (2024)           & $8959.06$   & $0.052$   & $0.xx$   & $0.xx$   & $98.712$ & $0.009$ & $0.xx$  & $0.xx$  \\
    MLP torch (2024)           & $0.xx$   & $0.xx$   & $0.xx$   & $0.xx$   & $0.xx$ & $0.xx$ & $0.xx$  & $0.xx$  \\
    MLP (2022)           & $4302.00^{\dagger}$  & n/a   & $7182.00^{\dagger}$   & n/a   & $864.00^{\dagger}$ & $0.008$ & foo & bar \\
    \\ 
    RFR (2024)                  & $0.562$   & $0.050$   & $0.016$   & $0.0007$   & $ 0.525$ &$0.015$ & foo & bar \\
    RFR (2022)                   & $0.559$   & $0.045 $   & $0.016$   & $0.0007$   & $ 0.528$ &$0.015 $ & foo & bar \\
   \\
    GPR sklearn (2024)     & $0.xx$ & $0.xx$   & $0.xx$ & $0.xx$ & $0.xx$ & $0.xx$ & foo & bar \\
    GPR GPflow (2024)     & $0.xx$ & $0.xx$   & $0.xx$ & $0.xx$ & $0.xx$ & $0.xx$ & foo & bar \\
    GPR (2022)     & $0.310$ & $0.019$   & $0.012$ & $0.0006$ & $0.306$ & $0.012$ & foo & bar \\
    \vspace{4pt}
%    \bottomrule
    \end{tabular}
    \caption{Elapsed time in seconds for model training and inference. Timing data from Wallace et al., 2022~\cite{wallace2022towards} does not have the same resolution as that of the current study and is shown in the format of $XX.YY^{\dagger}$, while other timing data is note available and shown as "n/a" in the table.}
    \label{tab:results_mse}
\end{table*}

